Beta Residuals: Improving Fault-Tolerant Control for Sensory Faults via Bayesian Inference and Precision Learning

Model-based fault-tolerant control (FTC) often consists of two distinct steps: fault detection & isolation (FDI), and fault accommodation. In this work we investigate posing fault-tolerant control as a single Bayesian inference problem. Previous work showed that precision learning allows for stochastic FTC without an explicit fault detection step. While this leads to implicit fault recovery, information on sensor faults is not provided, which may be essential for triggering other impact-mitigation actions. In this paper, we introduce a precision-learning based Bayesian FTC approach and a novel beta residual for fault detection. Simulation results are presented, supporting the use of beta residual against competing approaches.

==> tex/_reviews.tex <==
Reviewer 2 of Safeprocess 2022 submission 148

Comments to the author
======================

COMMENT: This paper describes an approach to fault-tolerant control
based on Bayesian inference, investigating taking control
action in a single step without an explicit fault detection
and reconfiguration which is a standard approach. The paper
is well written with clearly claimed contributions.

REPLY: thanks

COMMENT: The approach is based on sensor faults, as stated in the
introduction. This is limiting, can the approach be
extended to other types of faults? Otherwise, I think it
has to be compared to a sensor fault detection algorithm
combined with an alternative control approach not utilizing
the failed sensor.

REPLY: we can address this in a journal paper

COMMENT: The presentation is heavily based on Bayesian inference and
very little control (despite the title). For example, in
the concluding example, the results section, no control
performance plots are included. For me, the authors need to
more clearly connect to the underlying control problem they
claim to solve. This may require cutting down on the
Bayesian formalism they spend quite a lot of space on.
Further, there are multiple distribution assumptions made
in the approach (Gaussian, Gamma, Wishart, Ö) Arenít these
assumptions application dependent? In the simulation
example, is it possible to illustrate the sensitivity to
any assumptions?

REPLY: I agree, but again this can be fixed in a journal paper

COMMENT: In the Section VI, a 2-DOF robotic manipulator is studied
in a simulation study. I think it would be most useful for
the authors to include the full model equations. Judging by
equation (11) it is a simple linear model. Also, how many
sensors are included in the model? If there is only one, I
donít see how you can have recovery feedback control. On
the other hand, equation (11) indicates only one sensor.
Please clarify this. This way, a reader can evaluate the difficulty of the
problem. Now, it is easy to get lost in the Bayesian
formulations (I donít expect a full comparison with
competing approaches in a conference paper). I would like
to have a plot included where it is shown how the control
manages to recover a faulty sensor.


REPLY: We have no equation for the manipulator. Eq. (11) is not the dynamics indeed. @Mohamed can we add the equation for the manipulator?
There are three sensors, as stated at beginning of VI.A.
I do not think we have space for a plot where we see the controller recovering a fault. Maybe @Mohamed can you check if we can fit one plot?

In summary, an interesting paper but currently the authors
do not include enough information to evaluate the proposed
approach.

***

Reviewer 3 of Safeprocess 2022 submission 148

Comments to the author
======================

In summary, the manuscript proposed a reasonable method but
ignores the vast closely related literature on the general
approach. The presentation could also be improved. More
detailed comments are below.

1. The manuscript presents a Bayesian framework for FDI and
fault-tolerant control as being a completely new idea,
while ignoring the extensive literature on Bayesian
inference-based methods for FDI and fault-tolerant control,
which is found in any electronic search, e.g., a
GoogleScholar search of

fault detection Bayesian identification
fault detection Bayesian diagnosis
fault detection Bayesian isolation
fault-tolerance control Bayesian

That literature includes less restrictive formulations in
terms of the type of faults, and includes application to
real data collected from industry with industry coauthors,
as well as numerous academic case studies of various types.

Although there is a very large number of citations in the
manuscript, the manuscript does not draw any reasonable
connections to the most closely related publications on on
Bayesian inference-based methods for FDI and fault-tolerant
control. [The manuscript does cite one paper on the
Bayesian  approach to problems in stochastic estimation and
control which was published in 1964, ignores all subsequent
literature.]

Numerous publications discuss in detail the same points 
made in the introduction in the manuscript, and apply very
similar methodologies including the inference and
uncertainty quantification. Without drawing precise
connections to the most closely related publications, the
readers/reviewers are not provided with the information
needed to be able to accurately assess the novelty and
significance of the manuscript. Even reviewers like myself
who are familiar with that body of literature cannot
quickly find any differences between the method described
in the manuscript and the methods described in the
literature on this type of approach, because the literature
on Bayesian inference-based methods for FDI and
fault-tolerant control is so large and extensive. It is the
responsibility of the authors to provide that precise
information in the Introduction.

The large number of citations to weakly related
publications should be removed. There is no point in
restating what is already heavily discussed in the
literature, and instead focus on the most closely related
literature, and provide precise statements as to what is
different between the proposed method and the large number
of existing methods published in the literature, and
provide precise statements on the pros and cons between the
methods.

REPLY: I will rewrite part of the intro and cite many more papers, but the reviewer is missing the point that we are doing a different thing. They are requiring us to cite papers that are not related (except for the word Bayesian) and want us to remove literature that is related (but that they fail to see the relation with). So, just to be on the safe side, I will rewrite it.

Some papers I cite, and why:

"Bayesian Fault Detection and Diagnosis in Dynamic Systems"

This indeed includes a graphical probabilistic model (Dynamic Bayesian Network) and does inference using the same approach as a Kalman filter. They reduce the fault detection problem to tracking the system via a DBN. They do not design a threshold and do not recover faults (no control discussed)

"V. Verma, G. Gordon, R. Simmons and S. Thrun, "Real-time fault diagnosis [robot fault diagnosis]," in IEEE Robotics & Automation Magazine, vol. 11, no. 2, pp. 56-66, June 2004, doi: 10.1109/MRA.2004.1310942."

This one uses Particle Filters to track various fault hypotheses.

"P. Szolovits and S.G. Pauker, “Categorical and probabilistic reasoning in medical diagnosis revisited,” Artif. Intell., 1993."

This one is an historical paper on using Bayesian inference in a static way to relate symptoms to causes. No temporal relations.

"D. Codetta-Raiteri and L. Portinale, "Dynamic Bayesian Networks for Fault Detection, Identification, and Recovery in Autonomous Spacecraft," in IEEE Transactions on Systems, Man, and Cybernetics: Systems, vol. 45, no. 1, pp. 13-24, Jan. 2015, doi: 10.1109/TSMC.2014.2323212."

This shows that Probabilistic Graphic Models and DBN are applied to fault diagnosis of spacecrafts, but no mathematical details are provided. Mostly they talk about the implementation.

"Weike Sun, Antonio R.C. Paiva, Peng Xu, Anantha Sundaram, Richard D. Braatz,
Fault detection and identification using Bayesian recurrent neural networks,
Computers & Chemical Engineering,
Volume 141,
2020,"

This one I should have caught earlier, reviewer is right. It has several similitudes to our paper. Namely probabilistic approach, recursive inference over time (and space), variational approach to approximate posteriors. They propose either the squared Mahalanobis distance or the Local Distribution Ratio as a residual, for which the threshold is computed from the corresponding tail function. But, they need a Bayesian Recurrent Neural Network (our approach is simpler) and they do not include control.

"B. Cai, L. Huang, and M. Xie, “Bayesian Networks in Fault Diagnosis,” IEEE Trans. Ind. Inf., vol. 13, no. 5, pp. 2227–2240, Oct. 2017."

This is a survey we can briefly cite.



2. The writing quality could be improved. For example,

a. "In active fault tolerant techniques this output is used
to reconfigure the controller" is a run-on sentence.

b. "fault-detection" should be "fault detection" near the
end of Section 1.

c. "Model based fault-tolerant control" should be
"Model-based fault-tolerant control".

d. "non-linearities" should be "nonlinearities".

e. "false-positives" should be "false positives".

f. Something is wrong with the sentence, "These controllers
do not include component for FTC yet."

g. It is unclear why the dynamics of equation 1 are
referred to as being "following dynamics". The formulation
does not appear to be restricted to path-following or other
UAV or robotics problem. The general term for equation 1
would be "dynamics". Similarly, the manuscript repeatedly
referred to various nouns as being "following" when there
does not appear to be anything associated with the noun
that would be "following", and then "following" should be
deleted as conveying no information whatsoever.

h. "Sensory faults" should be "sensor faults".

i. The sentence "It also consistently outperform existing
methods on a variety of tasks." has a grammar error.

j. The extra parentheses in the equation in the 7th line up
from the bottom of Section II.B should be removed.

k. "one dimensional problems" should be "one-dimensional
problems".

l. "tr" should not be italicized.

m. Some parentheses are incorrectly sized.

n. The References have a large number of errors, including
in capitalization, in missing publisher city names for
books, missing page numbers, missing journal names, missing
volume numbers, and missing publisher names for books.

2. The manuscript needs to explicitly state that only
sensor faults -- by far the easiest type of fault -- are
considered in the manuscript. That restriction should be
explicitly stated in the title, abstract, introduction, and
conclusions.

3. The statement "It also consistently outperform existing
methods on a variety of tasks" is not shown in the
manuscript. Given the very large literature in this topic,
it is not possible for the authors to be able to state as a
fact that the method in this manuscript outperforms all
existing methods. At best, the manuscript could show that
the method outperforms the specific methods used for
comparison in the case study, and that would only be shown
for the specific case study.

4. The statement in Section II.C that the uncertainties in
state are usually not computed is wrong. The uncertainties
in the state are very commonly computed, and is the
foundation for the Kalman filter and other state
estimation-based approaches for process monitoring.

***

Reviewer 4 of Safeprocess 2022 submission 148

Comments to the author
======================

The paper my include publishable materials, and the
followings would help improve the quality of the paper:

1) Sensor noises are assumed to be zero mean Gaussian. The
reasonableness of the assumption should be clarified. 

2) The fault-tolerant approach is written in mathematical
way, which is hard for an engineer to follow. A
block-diagram would be helpful for the illustration. 

3) Only a figure is given for the simulation, which is
insufficient for the readers to understand the fault
diagnosis and fault tolerant control performance.  
